Some Problems in Compact Message Passing

This paper seeks to address the question of designing distributed algorithms for the setting of compact memory i.e. sublinear bits working memory for arbitrary connected networks. The nodes in our networks may have much lower internal memory as compared to the number of their possible neighbours implying that a node may not be able to store all the IDs of its neighbours. These algorithms are useful for large networks of small devices such as the Internet of Things, for wireless or ad-hoc networks, and, in general, as memory efficient algorithms. We introduce the Compact Message Passing(CMP) model;an extension of the standard message passing model considered at a finer granularity where a node can interleave reads and writes with internal computations, using a port only once in a round. The interleaving is required for meaningful computations due to the low memory requirement and is akin to a distributed network with nodes executing streaming algorithms. Note that the internal memory size upper bounds the message sizes and hence e.g. for log-memory, the model is weaker than the Congest model; for such models our algorithms will work directly too. We present early results in the CMP model for nodes with log^2-memory. We introduce the concepts of local compact functions and compact protocols and give solutions for some classic distributed problems (leader election, tree constructions and traversals). We build on these to solve the open problem of compact preprocessing for the compact self-healing routing algorithm CompactFTZ posed in Compact Routing Messages in Self-Healing Trees(TCS2017) by designing local compact functions for finding particular subtrees of labeled binary trees. Hence, we introduce the first fully compact self-healing routing algorithm. We also give independent fully compact versions of the Forgiving Tree[PODC08] and Thorup-Zwick's tree based compact routing[SPAA01].

==> relatedwork.tex <==
% !TEX root = LowMemCosher.tex

\subsection{Related work}

%This paper introduces the $\CModelAbbrev$ model formalizing the notion of sublinear (in number of nodes) memory.
 Earlier works have looked at various memory settings in distributed networks.
In~\protect\cite{EmekW13}, {Emek and Wattenhofer} study what can be computed in distributed manner using weak computational devices with constant local memory.
They introduce the \emph{network finite state machine} model in which weak nodes communicate in an asynchronous network. In every round of communication,
any node only broadcast a symbol taken from a constant size alphabet and
each time it reads its ports (all of them), only obtains the number of occurrences of each symbol up to some constant $d$,
namely, the node can only distinguish number of occurrences less or equal than $d$.
It is shown in~\protect\cite{EmekW13} that there are probabilisitic solutions to MST and 3-coloring of trees in this model.
In the \emph{beeping} model of communication~\protect\cite{DegesysRPN07}, nodes execute synchronous rounds, and in any round, each process decides to ``beep'' and send but not receive
or to stay silent and listen. A node that listens obtains a single bit encoding if at least one of its neighbours beeped in that round.
{Gilbert and Newport}~\protect\cite{GilbertN15} have shown that there are probabilistic solutions to the leader election problem in the beeping
model for the complete graph topology, in which each node is a state machine with constant states.
The aforementioned solutions in~\protect\cite{GilbertN15} imply compact probabilistic solution in our $\CModelAbbrev$ model.

As far as we know, the computational power of the CONGEST models ($O(poly \log n)$ sized messages)~\protect\cite{peleg} has never been studied when the local memory
of the nodes too is restricted. However, {Drucker et al.}~\protect\cite{DruckerKO13}  have studied the difference between nodes performing only broadcasts or doing unicast, showing that the unicast model is strictly more powerful.
{Becker et al.}~\protect\cite{BeckerARR15} have also studied the general case in which each node is restricted to sent a number of distinct messages in any round.

The concept of compact routing was pioneered by a number of well known papers {(Santoro and Khatib~\protect\cite{santoro1985labelling}, Peleg and Upfal~\protect\cite{PelegU88} and Cowen \protect\cite{Cowen01})}  trading stretch (factor increase in routing length) for memory used.
%The use of such routing protocols imposes only a constant factor increase in the length of the routing.
Several papers followed up with improvements on the schemes {(cf. Thorup and Zwick~\protect\cite{ThorupZ01}, Fraigniaud and Gavoille~\protect\cite{RoutingFraigniaudG01-short}, and Chechik~\protect\cite{Chechik13-short})}.
These schemes are made of two parts: a local preprocessing phase in which labels and routing tables are computed,
and a distributed phase in which the actual routing algorithm runs. Thus, these algorithms are in a sense not fully distributed but could be made distributed by making the preprocessing distributed.
Starting with~\protect\cite{AwerbuchBLP90, ElkinN16a, GavoilleGHI13, LenzenP13, LenzenP15}, there has been research on efficient implementations of the preprocessing phase in the CONGEST model (e.g.~\protect\cite{AwerbuchP92}).
However, these algorithms may not be compact (i.e. using $o(n)$ local memory)
even though the resulting routing scheme may be compact.
 Elkin and Neiman~\protect\cite{ElkinN17} claim a fully compact distributed routing algorithm using low memory in both the preprocessing and routing phases. However,~\protect\cite{ElkinN17} and related solutions are probabilistic. Our solution, on the other hand, is deterministic
 %, in a model of
 while also handling self-healing routing despite node failures, though we only handle tree based routing schemes in this work (unlike~\protect\cite{ElkinN17} etc).



Finally, dynamic network topology and fault tolerance are core concerns of distributed computing~\protect\cite{Attiya-WelchBook,Lynchbook} and various models, e.g.,~ \protect\cite{Kuhn-DistComputation-STOC10}, and topology maintenance and  self-* algorithms abound~\protect\cite{Berns09DissectingSelf-*,Djikstra74SelfStabilizing,DolevBookSelfStabilization,KormanKMPODC11,Kuhn2005Self-Repairing,Ghosh07Self-healingSystemsSurvey,  BeauquierBK-JThCS11, ElkinSpanners07, BaswanaSenSpanner-Icalp03, KuttenPorat-DynSPanningTree-DC99, COLLIN-DolevDFS, KuttenTrehanDFS2014}. The self-healing model was introduced in~\protect\cite{HayesPODC08,Amitabh-SelfHeal-arxiv} leading to a variety of self-healing topology maintenance algorithms~\protect\cite{Pandurangan2014-DEX, PanduranganXhealT14, FG-DCJournal2012, Amitabh-2010-PhdThesis, SarmaTrehanEdgeNetSciComm2012,SaiaTrehanIPDPS08}. $\cft$~\protect\cite{CDT2018-CompactFTZ} is a compact variant of the ForgivingTree~\protect\cite{HayesPODC08}. One of the central techniques used in these topological self-healing algorithms is the concept of a reconstruction structure based on graph families such as balanced binary search trees~\protect\cite{HayesPODC08}, half-full trees~\protect\cite{FG-DCJournal2012}, random r-regular expanders~\protect\cite{PanduranganXhealT14}, and p-cycle deterministic expanders in~\protect\cite{Pandurangan2014-DEX}. Of particular interest is the half-full tree for which we derive a compact function in this paper.

